Frictional Agent Alignment Framework: Slow Down and Don't Break Things

AI support of collaborative interactions entails mediating potential misalignment between interlocutor beliefs. Common preference alignment methods like DPO excel in static settings, but struggle in dynamic collaborative tasks where the explicit signals of interlocutor beliefs are sparse and skewed. We propose the Frictional Agent Alignment Framework (FAAF), to generate precise, context-aware "friction" that prompts for deliberation and re-examination of existing evidence. FAAF's two-player objective decouples from data skew: a frictive-state policy identifies belief misalignments, while an intervention policy crafts collaborator-preferred responses. We derive an analytical solution to this objective, enabling training a single policy via a simple supervised loss. Experiments on three benchmarks show FAAF outperforms competitors in producing concise, interpretable friction and in OOD generalization. By aligning LLMs to act as adaptive "thought partners" -- not passive responders -- FAAF advances scalable, dynamic human-AI collaboration. Our code and data can be found at https://github.com/csu-signal/FAAF_ACL.

==> deli_wtd_opt_rm_pairwise_results.tex <==
\begin{table*}[t]

\centering
\small
\begin{tabular}{llccccc}
 \toprule
        & & \multicolumn{5}{c}{\textbf{Win-rates}} \\
        \cmidrule(lr){3-7}
        \textbf{Dataset} & \textbf{Policy} & vs. Base & vs. SFT & vs. DPO & vs. IPO & vs. PPO \\
        %\cmidrule(lr){3-7}
 
        \midrule
        \multirow{}{DeliData} 

        
        & \texttt{FAAF}$_{\Delta R'}$    & 0.822$_{\pm 0.017}$ & 0.788$_{\pm 0.018}$ & 0.740$_{\pm 0.019}$ & 0.536$_{\pm 0.022}$ & 0.792$_{\pm 0.018}$ \\

        
        & \texttt{FAAF}$_{\Delta R}$    & 0.858$_{\pm 0.015}$ & 0.814$_{\pm 0.017}$ & 0.732
$_{\pm 0.019}$ & 0.542
$_{\pm 0.022}$ & 0.734$_{\pm 0.019}$ \\
        
       & \texttt{FAAF}$_{\Delta(R+R')}$ & 0.862$_{\pm 0.015}$ & 0.84
$_{\pm 0.016}$ & 0.756$_{\pm 0.019}$ & 0.796$_{\pm 0.018}$ & 0.76$_{\pm 0.019}$ \\


        
        \midrule
        \multirow{}{WTD Sim.} 
        & \texttt{FAAF}$_{\Delta R'}$   & 0.791$_{\pm 0.019}$ & 0.802$_{\pm 0.018}$ & 0.704$_{\pm 0.021}$ & 0.686$_{\pm 0.021}$ & 0.608$_{\pm 0.023}$ \\

        
        & \texttt{FAAF}$_{\Delta R}$   & 0.857$_{\pm 0.016}$ & 0.808$_{\pm 0.018}$ & 0.708$_{\pm 0.021}$ & 0.722$_{\pm 0.021}$ & 0.748$_{\pm 0.020}$ \\


        
     & \texttt{FAAF}$_{\Delta(R+R')}$ & 0.88$_{\pm 0.015}$ & 0.837$_{\pm 0.017}$ & 0.728$_{\pm 0.020}$ & 0.737$_{\pm 0.020}$ & 0.751$_{\pm 0.020}$ \\




        
        \midrule
        \multirow{}{WTD Orig.} 
        & \texttt{FAAF}$_{\Delta R'}$   & 0.78$_{\pm 0.058}$ & 0.78$_{\pm 0.058}$ & 0.76$_{\pm 0.060}$ & 0.58$_{\pm 0.069}$ & 0.58$_{\pm 0.069}$ \\


        
        & \texttt{FAAF}$_{\Delta R}$   & 0.68$_{\pm 0.065}$ & 0.74$_{\pm 0.062}$ & 0.54$_{\pm 0.070}$ & 0.62$_{\pm 0.068}$ & 0.70$_{\pm 0.064}$ \\


        
      & \texttt{FAAF}$_{\Delta(R+R')}$ & 0.84$_{\pm 0.051}$ & 0.76$_{\pm 0.060}$ & 0.74$_{\pm 0.062}$ & 0.74$_{\pm 0.062}$ & 0.82$_{\pm 0.054}$ \\
        \bottomrule
\end{tabular}
\caption{Ablation study comparing FAAF variants against baseline methods in pairwise comparisons. All experiments use \texttt{Meta-Llama-3-8B-Instruct} (temperature 0.7, top-p 0.9). Baselines include SFT-initialized DPO~\citep{rafailov2024direct}, IPO~\citep{azar2024general}, and PPO~\citep{schulman2017proximal}. We compare three FAAF variants: FAAF$_{\Delta R'}$ (unconditioned), FAAF$_{\Delta R}$ (with $\phi$-conditioning), and FAAF$_{\Delta(R+R')}$ (full objective), reporting win rates ($\pm$ std) for each comparison.}


\label{tab:opt_rm_performance_comparison}
\end{table*}


==> faaf_pseudo_code.tex <==
\begin{figure*}[h!]
\lstset{
    backgroundcolor=\color{white},
    basicstyle=\ttfamily\small\color{black},
    keywordstyle=\color{blue}\bfseries,
    commentstyle=\color{gray}\itshape,
    stringstyle=\color{orange},
    numberstyle=\tiny\color{gray},
    rulecolor=\color{black},
    frame=single,
    breaklines=true,
    tabsize=4,
    captionpos=b,
    language=Python
}
\begin{lstlisting}[language=Python, frame=none]
import torch
def faaf_loss(policy_chosen_logps, policy_rejected_logps,        # π_θ(f_w|φ,x), π_θ(f_l|φ,x)
              reference_chosen_logps, reference_rejected_logps,   # π_ref(f_w|φ,x), π_ref(f_l|φ,x)
              policy_chosen_friction_logps,                       # π_θ(f_w|x)
              policy_rejected_friction_logps,                     # π_θ(f_l|x)
              reference_chosen_friction_logps,                    # π_ref(f_w|x)
              reference_rejected_friction_logps,                  # π_ref(f_l|x)
              beta):
    '''
    Compute FAAF loss combining conditional and unconditioned policy ratios
    with friction-aware preference alignment.
    '''
    # Compute conditional policy log ratios (ΔR term)
    pi_logratios = policy_chosen_logps - policy_rejected_logps
    ref_logratios = reference_chosen_logps - reference_rejected_logps
    logits = pi_logratios - ref_logratios

    # Compute unconditioned policy log ratios (ΔR' term)
    pi_friction_logratios = policy_chosen_friction_logps - policy_rejected_friction_logps
    ref_friction_logratios = reference_chosen_friction_logps - reference_rejected_friction_logps
    friction_only_logits = pi_friction_logratios - ref_friction_logratios

    # Compute FAAF loss with both reward differences
    losses = (beta * (logits + friction_only_logits) - 1/2)**2

    # Compute rewards for monitoring (detached)
    chosen_rewards = beta * (policy_chosen_logps - reference_chosen_logps).detach()
    rejected_rewards = beta * (policy_rejected_logps - reference_rejected_logps).detach()
    chosen_friction_rewards = beta * (policy_chosen_friction_logps - reference_chosen_friction_logps).detach()
    rejected_friction_rewards = beta * (policy_rejected_friction_logps - reference_rejected_friction_logps).detach()

    return losses, chosen_rewards, rejected_rewards, chosen_friction_rewards, rejected_friction_rewards
\end{lstlisting}
\caption{FAAF Objective with minimal PyTorch implementation. The loss combines two reward difference terms: conditional policy ratios ($\Delta R$) and unconditioned policy ratios ($\Delta R'$) for friction-aware preference alignment.}
\label{fig:faaf_implementation_pytorch}
\end{figure*}

==> friction_eval_prompt.tex <==
\begin{figure*}[hbtp] % Use figure* for spanning across both columns
    \centering
    \begin{adjustbox}{width=1.8\textwidth}  % Make it cover the full two-column width
    \lstset{
        basicstyle=\ttfamily\small,  % Set font size to small
        breaklines=true,
        frame=none,
        language=json
    }
    \begin{lstlisting}[frame=none]
Please evaluate the following friction intervention and rationale according to these criteria:

*Relevance (1-5)*: How well does the intervention address key issues or assumptions in the reasoning process?
1 = Not at all relevant
3 = Somewhat relevant
5 = Extremely relevant

*Specificity (1-5)*: Does the intervention pinpoint specific flaws, assumptions, or gaps?
1 = Very general suggestions
3 = Mix of specific and general
5 = Highly specific and targeted

*Clarity (1-5)*: Is the intervention clear, concise, and easy to understand?
1 = Very unclear and ambiguous
3 = Moderately clear
5 = Extremely clear and easy to understand

*Rationale Alignment (1-5)*: How well does the rationale align with and justify the intervention preference?
1 = Rationale does not align at all
3 = Rationale somewhat aligns
5 = Rationale strongly aligns and justifies preference

*Actionability (1-5)*: Does the intervention provide actionable guidance or concrete steps to improve reasoning?
1 = No actionable guidance
3 = Some actionable suggestions
5 = Clear and concrete steps for improvement

*Potential Consequence (1-5)*: To what extent could the intervention change the course of reasoning for the better or worse to help the group's task completion?
1 = Unlikely to have any significant impact
3 = Moderate potential for impact
5 = High potential to significantly alter reasoning

*Helpfulness (1-5)*: Overall, how helpful is this intervention likely to be for improving the reasoning process?
1 = Not at all helpful
3 = Somewhat helpful
5 = Extremely helpful

**Friction Intervention**: "{intervention}"
**Rationale**: "{rationale}"

**Scores**:
Relevance: {relevance_score}
Specificity: {specificity_score}
Clarity: {clarity_score}
Rationale Alignment: {rationale_alignment_score}
Actionability: {actionability_score}
Potential Consequence: {potential_consequence_score}
Helpfulness: {helpfulness_score}
    \end{lstlisting}
    \end{adjustbox}
    \caption{Evaluation prompt used for friction intervention assessments. This prompt systematically scores interventions based on clarity, specificity, rationale alignment, and overall helpfulness. It follows structured evaluation criteria similar to previous AI alignment methods~\cite{rafailov2024direct}. The final scores determine the effectiveness of different intervention strategies.}
    \label{fig:friction_eval_prompt}
\end{figure*}


==> human_eval_prompt.tex <==
\begin{tcolorbox}[title=Friction Intervention Rating Survey]
Given two intervention choices A and B, please rate each on a scale of 1-5 (1=Poor, 5=Excellent) across the following dimensions:

\begin{enumerate}
\item \textbf{Relevance} (1-5): Does the intervention target key reasoning issues?
\item \textbf{Gold Alignment} (1-5): How well does it match the gold standard friction?
\item \textbf{Actionability} (1-5): Does it provide concrete steps for improvement?
\item \textbf{Rationale Fit} (1-5): Is the rationale well-aligned with the intervention?
\item \textbf{Thought-Provoking} (1-5): Does it encourage meaningful reflection?
\item \textbf{Specificity} (1-5): Does it identify precise flaws or gaps?
\item \textbf{Impact} (1-5): Can it effectively change reasoning trajectory?
\item \textbf{Clarity} (1-5): Is it clear and easily understood?
\end{enumerate}

\textbf{Response Format:}
\begin{verbatim}
A: {
  relevance: [1-5],         gold_alignment: [1-5],
  actionability: [1-5],     rationale_fit: [1-5],
  thought_provoking: [1-5], specificity: [1-5],
  impact: [1-5],           clarity: [1-5]
}

B: {
  [Same format as A]
}

Winner: ['A' or 'B']
Rationale: [One sentence explanation for choice]
\end{verbatim}
\end{tcolorbox}

==> rough_notes.tex <==
Notice that although we have analytically derived two specific formulations---optimal  frictive-state policy ($ \pi_\phi^*(\phi|x)$) and the optimal \textit{unconditioned} friction-agent policy ($\pi_\phi^*(f|x)$) derived above--clearly, $\pi_\phi^*(f|x)$ has no information of the beliefs since it does not depend on the frictive-state. As defined in our FAAF optimization objective, the friction agent is explicitly conditioned on $\phi$, and this is the policy we care about. However, note that we have already derived the formulation of this policy (as $\pi_f^*(f \mid \phi, x) = \frac{\exp\left(\frac{p(f \succ \phi \mid x)}{\beta}\right) \pi_{\text{ref}}(f \mid \phi, x)}{Z^*(\phi, x)}$
) in the inner maximimization objective (Eq. \ref{eq:optimal_friction_inner_max_solution}). 


% \begin{theorem}[Optimality Properties]
% The derived optimal frictive policy $\pi_\phi^*$ satisfies three key properties:
% \begin{enumerate}
%     \item It maintains proportionality with the reference policy $\pi_{ref}$.
%     \item It assigns lower probability to states with higher improvement potential, modulated by $Z^*(\phi, x)$.
%     \item It ensures proper normalization through the partition function $Z(x)$.
% \end{enumerate}
% \end{theorem}



%initial objective derivation


  
Now, we can represent the log-ratios of both these policies derived in Eq.\ref{eq:optimal_frictive_state_policy} and Eq.\ref{eq:optimal_frictive_agent_policy_unconditioned} wrt to their reference policies as shown below: 

\begin{align*}
\log\Big(\frac{\pi_\phi^*(\phi|x)}{\pi_{ref}(\phi|x)}\Big) &= -\log(Z^*(\phi,x)) - \log(Z^*(x)) \\
\log\Big(\frac{\pi_\phi^*(f|x)}{\pi_{ref}(f|x)}\Big) &= -\log(Z^*(f,x)) - \log(Z^*(x))
\end{align*}

\begin{align}
p(f \succ \phi|x) 
&= \beta \Big[\log(\pi_f^*(f|\phi,x)) - \log(\pi_{ref}(f|\phi,x)) 
+ \frac{1}{2\beta} - (-\log(Z^*(\phi,x)) - \log(Z^*(x))) \notag \\
&\quad + (-\log(Z^*(f,x)) - \log(Z^*(x))) \Big] \notag \\
&= \beta \Big[\log(\pi_f^*(f|\phi,x)) - \log(\pi_{ref}(f|\phi,x)) 
+ \log(Z^*(\phi,x)) \\
& + \log(Z^*(x)) - \log(Z^*(f,x)) - \log(Z^*(x)) \Big] 
+ \frac{1}{2} \notag \\
&= \beta \Big[\log(\pi_f^*(f|\phi,x)) - \log(\pi_{ref}(f|\phi,x)) 
+ \log(Z^*(\phi,x)) - \log(Z^*(f,x)) \Big] + \frac{1}{2} \notag \\
&= \beta \Big[\log(\pi_f^*(f|\phi,x)) - \log(\pi_{ref}(f|\phi,x)) 
- \log \Big(\frac{\pi_\phi^*(\phi|x)}{\pi_{ref}(\phi|x)}\Big) 
+ \log \Big(\frac{\pi_\phi^*(f|x)}{\pi_{ref}(f|x)}\Big) \Big] + \frac{1}{2} \notag \\
&= \frac{1}{2} + \frac{\beta}{2} \Big[\log \Big(\frac{\pi_f^*(f|\phi,x)}{\pi_{ref}(f|\phi,x)}\Big) 
- \log \Big(\frac{\pi_\phi^*(\phi|x)}{\pi_{ref}(\phi|x)}\Big) 
- \log \Big(\frac{\pi_f^*(\phi|f,x)}{\pi_{ref}(\phi|f,x)}\Big) 
+ \log \Big(\frac{\pi_\phi^*(f|x)}{\pi_{ref}(f|x)}\Big) \Big].
\label{eq:final_four_term_preference_expression}
\end{align}

We begin with the four-term preference expression 
\begin{equation}
\begin{split}
p(f \succ \phi|x) = \frac{1}{2} + \frac{\beta}{2}&\Big[\log\Big(\frac{\pi_f^*(f|\phi,x)}{\pi_{ref}(f|\phi,x)}\Big) - \log\Big(\frac{\pi_\phi^*(\phi|x)}{\pi_{ref}(\phi|x)}\Big) \\  
&- \log\Big(\frac{\pi_f^*(\phi|f,x)}{\pi_{ref}(\phi|f,x)}\Big) + \log\Big(\frac{\pi_\phi^*(f|x)}{\pi_{ref}(f|x)}\Big)\Big]
\end{split}
\end{equation}
 
\begin{step}[Combine terms]
After substituting and collecting terms:
\begin{align*}
p(f \succ \phi|x) = \frac{1}{2} + \frac{\beta}{2}&\Big[\log\Big(\frac{\pi_f^*(f|\phi,x)}{\pi_{ref}(f|\phi,x)}\Big) - \log\Big(\frac{\pi_\phi^*(\phi|x)}{\pi_{ref}(\phi|x)}\Big) \\
&- \log\Big(\frac{\pi_f^*(\phi|f,x)}{\pi_{ref}(\phi|f,x)}\Big) + \log\Big(\frac{\pi_\phi^*(f|x)}{\pi_{ref}(f|x)}\Big)\Big]
\end{align*}
\end{step}


We begin with the four-term preference expression:
\begin{equation}
\begin{split}
p(f \succ \phi|x) = \frac{1}{2} + \frac{\beta}{2}&\Big[\log\Big(\frac{\pi_f^*(f|\phi,x)}{\pi_{ref}(f|\phi,x)}\Big) - \log\Big(\frac{\pi_\phi^*(\phi|x)}{\pi_{ref}(\phi|x)}\Big) \\
&- \log\Big(\frac{\pi_f^*(\phi|f,x)}{\pi_{ref}(\phi|f,x)}\Big) + \log\Big(\frac{\pi_\phi^*(f|x)}{\pi_{ref}(f|x)}\Big)\Big]
\end{split}
\end{equation}

\begin{step}[Empirical Preference Substitution]
For a preferred friction response $f_w$ over a less preferred frictive state $\phi_l$:
\begin{equation}
p(f_w \succ \phi_l|x) = 1
\end{equation}
\end{step}

\begin{step}[Substitution and Rearrangement]
Substituting the empirical preference:
\begin{equation}
\begin{split}
1 = \frac{1}{2} + \frac{\beta}{2}&\Big[\log\Big(\frac{\pi_f^*(f_w|\phi_l,x)}{\pi_{ref}(f_w|\phi_l,x)}\Big) - \log\Big(\frac{\pi_\phi^*(\phi_l|x)}{\pi_{ref}(\phi_l|x)}\Big) \\
&- \log\Big(\frac{\pi_f^*(\phi_l|f_w,x)}{\pi_{ref}(\phi_l|f_w,x)}\Big) + \log\Big(\frac{\pi_\phi^*(f_w|x)}{\pi_{ref}(f_w|x)}\Big)\Big]
\end{split}
\end{equation}
\end{step}

\begin{step}[Multiply by 2]
\begin{equation}
\begin{split}
2 = 1 + \beta&\Big[\log\Big(\frac{\pi_f^*(f_w|\phi_l,x)}{\pi_{ref}(f_w|\phi_l,x)}\Big) - \log\Big(\frac{\pi_\phi^*(\phi_l|x)}{\pi_{ref}(\phi_l|x)}\Big) \\
&- \log\Big(\frac{\pi_f^*(\phi_l|f_w,x)}{\pi_{ref}(\phi_l|f_w,x)}\Big) + \log\Big(\frac{\pi_\phi^*(f_w|x)}{\pi_{ref}(f_w|x)}\Big)\Big]
\end{split}
\end{equation}
\end{step}

\begin{step}[Subtract 1]
\begin{equation}
\begin{split}
1 = \beta&\Big[\log\Big(\frac{\pi_f^*(f_w|\phi_l,x)}{\pi_{ref}(f_w|\phi_l,x)}\Big) - \log\Big(\frac{\pi_\phi^*(\phi_l|x)}{\pi_{ref}(\phi_l|x)}\Big) \\
&- \log\Big(\frac{\pi_f^*(\phi_l|f_w,x)}{\pi_{ref}(\phi_l|f_w,x)}\Big) + \log\Big(\frac{\pi_\phi^*(f_w|x)}{\pi_{ref}(f_w|x)}\Big)\Big]
\end{split}
\end{equation}
\end{step}

\begin{observation}[Optimality Condition]
For optimal policies, the following consistency condition holds:
\begin{equation}
\log\Big(\frac{\pi_\phi^*(\phi_l|x)}{\pi_{ref}(\phi_l|x)}\Big) + \log\Big(\frac{\pi_f^*(\phi_l|f_w,x)}{\pi_{ref}(\phi_l|f_w,x)}\Big) \approx 0
\end{equation}

This holds because optimal policies should be consistent in their evaluation of the less preferred option $\phi_l$.
\end{observation}

\begin{step}[Apply Optimality Condition]
After applying the optimality condition:
\begin{equation}
1 = \beta\Big[\log\Big(\frac{\pi_f^*(f_w|\phi_l,x)}{\pi_{ref}(f_w|\phi_l,x)}\Big) + \log\Big(\frac{\pi_\phi^*(f_w|x)}{\pi_{ref}(f_w|x)}\Big)\Big]
\end{equation}
\end{step}

\begin{step}[Replace with Trainable Model]
For our trainable model $\pi$, we replace $\pi^*$ with $\pi$:
\begin{equation}
1 = \beta\Big[\log\Big(\frac{\pi(f_w|\phi_l,x)}{\pi_{ref}(f_w|\phi_l,x)}\Big) + \log\Big(\frac{\pi(f_w|x)}{\pi_{ref}(f_w|x)}\Big)\Big]
\end{equation}
\end{step}

\begin{step}[Final Loss Function]
The practical loss is the squared error between predicted and true preference:
\begin{equation}
L_b(\pi) = \mathbb{E}_{(\phi_l,f_w,x)\sim D}\Big[\Big(\beta\Big[\log\Big(\frac{\pi(f_w|\phi_l,x)}{\pi_{ref}(f_w|\phi_l,x)}\Big) + \log\Big(\frac{\pi(f_w|x)}{\pi_{ref}(f_w|x)}\Big)\Big] - 1\Big)^2\Big]
\end{equation}
\end{step}



final proof steps 


Substituting this back into Eq.~\ref{eq:preference_prob_friction_over_frictive_state} results in:
\begin{align}
p(f \succ \phi|x) 
&= \beta[\log(\pi_f^*(f|\phi,x)) - \log(\pi_{ref}(f|\phi,x)) \notag \\
&\quad + \frac{1}{2\beta} - (\log(\pi_f^*(\phi|\phi,x)) - \log(\pi_{ref}(\phi|\phi,x)))] \notag \\
&= \beta \log \left( \frac{\pi_f^*(f|\phi,x)}{\pi_{ref}(f|\phi,x)} \right) 
+ \frac{1}{2} 
- \beta \log \left( \frac{\pi_f^*(\phi|\phi,x)}{\pi_{ref}(\phi|\phi,x)} \right).
\label{eq:identity_optimal_conditioned_ratios}
\end{align}

The $\log ( \frac{\pi_f^*(\phi|\phi,x)}{\pi_{ref}(\phi|\phi,x)}$ term in the above step is a self-referential term signifying the friction intervention policy's ($\pi_f^*(\cdot \mid \phi, x)$) estimate of the frictive-state $\phi$ given $\phi$. However, this term does \textit{not} provide much information on the regularized preference in terms of the frictive state policy. Recall that our outer minimization objective operates over $ \pi_\phi(\cdot|x)$. \textcolor{blue}{Fortunately, we can use our results from \Cref{theorem:threshold_theorem_sequential_choice} and \Cref{lemma:policy_ratio_equivalence} to express \Cref{eq:identity_optimal_conditioned_ratios} in terms of  the optimal frictive state policy $\pi_\phi^*(\cdot|x)$. Therefore, from \Cref{lemma:policy_ratio_equivalence} we can express $\pi_f^*$ and $\pi_{\text{ref}}$ as follows: }

For the optimal policy $\pi_f^*$:
\begin{align}
\log(\pi_f^*(\phi|\phi,x)) &= \log(\pi_\phi^*(\phi|x)) - \log(\pi_\phi^*(f|x))
\end{align}

For the reference policy $\pi_{\text{ref}}$:
\begin{align}
\log(\pi_{\text{ref}}(\phi|\phi,x)) &= \log(\pi_{\text{ref}}(\phi|x)) - \log(\pi_{\text{ref}}(f|x))
\end{align}

Now, substituting these expressions into \Cref{eq:identity_optimal_conditioned_ratios}, we get:
\begin{align}
p(f \succ \phi|x) 
&= \beta \Big[\log(\pi_f^*(f|\phi,x)) - \log(\pi_{\text{ref}}(f|\phi,x)) 
+ \frac{1}{2\beta} - \log(\pi_\phi^*(\phi|x)) \notag \\
&\quad + \log(\pi_\phi^*(f|x)) - \log(\pi_{\text{ref}}(\phi|x)) 
+ \log(\pi_{\text{ref}}(f|x)) \Big] \notag \\
&= \beta \Big[\log(\pi_f^*(f|\phi,x)) - \log(\pi_{\text{ref}}(f|\phi,x)) 
+ \frac{1}{2\beta} - \Big(\log(\pi_\phi^*(\phi|x)) - \log(\pi_{\text{ref}}(\phi|x)) \notag \\
&\quad - (\log(\pi_\phi^*(f|x)) - \log(\pi_{\text{ref}}(f|x)))\Big)\Big] \notag \\
&= \beta\Bigg[\log\left(\frac{\pi_f^*(f|\phi,x)}{\pi_{\text{ref}}(f|\phi,x)}\right) + \frac{1}{2\beta} 
+ \log\left(\frac{\pi_f^*(f|x)}{\pi_{\text{ref}}(f|x)}\right) \notag \\
&\quad - \log\left(\frac{\pi_f^*(\phi|x)}{\pi_{\text{ref}}(\phi|x)}\right)\Bigg].
\end{align}



Now, replacing $f$ by $f_1$ in $p(f \succ \phi|x)$:
\begin{align}
p(f_1 \succ \phi|x) &= \beta\Bigg[\log\left(\frac{\pi_f^*(f_1|\phi,x)}{\pi_{\text{ref}}(f_1|\phi,x)}\right) + \frac{1}{2\beta} + \log\left(\frac{\pi_f^*(f_1|x)}{\pi_{\text{ref}}(f_1|x)}\right) \notag \\
&\quad - \log\left(\frac{\pi_f^*(\phi|x)}{\pi_{\text{ref}}(\phi|x)}\right)\Bigg]
\end{align}

Similarly, expressing $f_2$ in $p(f \succ \phi|x) $, we obtain: 
\begin{align}
p(f_2 \succ \phi|x) &= \beta\Bigg[\log\left(\frac{\pi_f^*(f_2|\phi,x)}{\pi_{\text{ref}}(f_2|\phi,x)}\right) + \frac{1}{2\beta} + \log\left(\frac{\pi_f^*(f_2|x)}{\pi_{\text{ref}}(f_2|x)}\right) \notag \\
&\quad - \log\left(\frac{\pi_f^*(\phi|x)}{\pi_{\text{ref}}(\phi|x)}\right)\Bigg]
\end{align}

Now, expressing $p(f_1 \succ \phi|x) - p(f_2 \succ \phi|x)$, the relative preference probability of $f_1$ over $f_2$ given $\phi$ and $x$,  we observe that $\log\left(\frac{\pi_f^*(\phi|x)}{\pi_{\text{ref}}(\phi|x)}\right)$ terms cancel out and we derive:


\begin{align}
&p(f_1 \succ \phi|x) - p(f_2 \succ \phi|x) = \\
&\beta\Bigg[\log\left(\frac{\pi_f^*(f_1|\phi,x)}{\pi_{\text{ref}}(f_1|\phi,x)}\right) + \frac{1}{2\beta} + \log\left(\frac{\pi_f^*(f_1|x)}{\pi_{\text{ref}}(f_1|x)}\right) - \log\left(\frac{\pi_f^*(\phi|x)}{\pi_{\text{ref}}(\phi|x)}\right)\Bigg] \notag \\
&- \beta\Bigg[\log\left(\frac{\pi_f^*(f_2|\phi,x)}{\pi_{\text{ref}}(f_2|\phi,x)}\right) + \frac{1}{2\beta} + \log\left(\frac{\pi_f^*(f_2|x)}{\pi_{\text{ref}}(f_2|x)}\right) - \log\left(\frac{\pi_f^*(\phi|x)}{\pi_{\text{ref}}(\phi|x)}\right)\Bigg] \notag \\
&= \beta\Bigg[\log\left(\frac{\pi_f^*(f_1|\phi,x)}{\pi_{\text{ref}}(f_1|\phi,x)}\right) - \log\left(\frac{\pi_f^*(f_2|\phi,x)}{\pi_{\text{ref}}(f_2|\phi,x)}\right) \notag \\
&\quad + \log\left(\frac{\pi_f^*(f_1|x)}{\pi_{\text{ref}}(f_1|x)}\right) - \log\left(\frac{\pi_f^*(f_2|x)}{\pi_{\text{ref}}(f_2|x)}\right)\Bigg]
\end{align}

\textcolor{red}{This above result is one of our \textit{core contributions} since it lets us express the preference of any friction intervention $f_1$ over $f_2$ given a frictive-state $\phi$ and the context, $x$ analytically in terms of \textbf{both} the friction intervention policy and the frictive-state policy.}


\begin{align}
p(f_1 \succ \phi|x) - p(f_2 \succ \phi|x) &= \beta\Bigg[\log\left(\frac{\pi_f^*(f_1|\phi,x)}{\pi_{\text{ref}}(f_1|\phi,x)}\right) - \log\left(\frac{\pi_f^*(f_2|\phi,x)}{\pi_{\text{ref}}(f_2|\phi,x)}\right) \notag \\
&\quad + \log\left(\frac{\pi_f^*(f_1|x)}{\pi_{\text{ref}}(f_1|x)}\right) - \log\left(\frac{\pi_f^*(f_2|x)}{\pi_{\text{ref}}(f_2|x)}\right)\Bigg]
\end{align}


To learn the optimal friction intervention policy $\pi_f^*$, we parametrize it using learnable parameters $\theta$ and train $\pi_\theta$ through the following $\ell_2$ loss that enforces the relative preference ordering between any pair of friction interventions $(f_1, f_2)$:

\begin{align}
\mathcal{L}_{\pi_\theta} = \mathbb{E}_{\substack{x \sim \rho \\ \phi \sim \pi_\theta(\cdot|x) \\ f_1,f_2 \sim \pi_\theta(\cdot|\phi,x)}} 
&\Bigg(p(f_1 \succ \phi|x) - p(f_2 \succ \phi|x) - \notag \\
&\beta\Bigg[\log\left(\frac{\pi_\theta(f_1|\phi,x)}{\pi_{\text{ref}}(f_1|\phi,x)}\right) - \log\left(\frac{\pi_\theta(f_2|\phi,x)}{\pi_{\text{ref}}(f_2|\phi,x)}\right) \notag \\
&\quad + \log\left(\frac{\pi_\theta(f_1|x)}{\pi_{\text{ref}}(f_1|x)}\right) - \log\left(\frac{\pi_\theta(f_2|x)}{\pi_{\text{ref}}(f_2|x)}\right)\Bigg]\Bigg)^2
\end{align}

Since the friction dataset $\mathcal{D}$ contains preference-annotated pairs $(f_w, f_l)$ given $\phi$ and $x$, the preference probabilities can be expressed using indicator functions as $p(f_w \succ f_l|x) = \mathbb{E}[\mathbbm{1}(f_w \succ f_l|x)] = 1$ and $p(f_l \succ f_w|x) = \mathbb{E}[\mathbbm{1}(f_l \succ f_w|x)] = 0$. Furthermore, the difference $p(f_w \succ f_l|x) - p(f_l \succ f_w|x) = 1 - 0 = 1$ aligns with the formulation $p(f_1 \succ \phi|x) - p(f_2 \succ \phi|x)$ when $f_1 = f_w$ and $f_2 = f_l$. \textcolor{blue}{Therefore, we can write our final FAAF-alignment empirical objective function ($\hat{\mathcal{L}}$) as follows:}

\begin{align}
\hat{\mathcal{L}} (\pi_\theta) = \mathbb{E}_{(x,\phi,f_w,f_l) \sim \mathcal{D}} 
&\Bigg(1 - \beta\Bigg[\log\left(\frac{\pi_\theta(f_w|\phi,x)}{\pi_{\text{ref}}(f_w|\phi,x)}\right) \notag \\
&- \log\left(\frac{\pi_\theta(f_l|\phi,x)}{\pi_{\text{ref}}(f_l|\phi,x)}\right) 
+ \log\left(\frac{\pi_\theta(f_w|x)}{\pi_{\text{ref}}(f_w|x)}\right) \notag \\
&- \log\left(\frac{\pi_\theta(f_l|x)}{\pi_{\text{ref}}(f_l|x)}\right)\Bigg]\Bigg)^2
\end{align}

where $(f_w, f_l)$ represent the winning (preferred) and losing (less preferred) friction interventions respectively in each annotated pair.

\begin{align}
\hat{\mathcal{L}} (\pi_\theta) = \mathbb{E}_{(x,\phi,f_w,f_l) \sim \mathcal{D}} 
&\Bigg(1 - \beta\Bigg[\log\left(\frac{\pi_\theta(f_w|\phi,x)\pi_{\text{ref}}(f_l|\phi,x)}{\pi_\theta(f_l|\phi,x)\pi_{\text{ref}}(f_w|\phi,x)}\right) \notag \\
&+ \log\left(\frac{\pi_\theta(f_w|x)\pi_{\text{ref}}(f_l|x)}{\pi_\theta(f_l|x)\pi_{\text{ref}}(f_w|x)}\right)\Bigg]\Bigg)^2
\end{align}

\begin{align}
\hat{\mathcal{L}} (\pi_\theta) = \mathbb{E}_{(x,\phi,f_w,f_l) \sim \mathcal{D}}  \Bigg(1 - \beta\Bigg[\underbrace{\log\left(\frac{\pi_\theta(f_w|\phi,x)\pi_{\text{ref}}(f_l|\phi,x)}{\pi_\theta(f_l|\phi,x)\pi_{\text{ref}}(f_w|\phi,x)}\right)}_{reward~difference} + \underbrace{\log\left(\frac{\pi_\theta(f_w|x)\pi_{\text{ref}}(f_l|x)}{\pi_\theta(f_l|x)\pi_{\text{ref}}(f_w|x)}\right)}_{reward~difference}\Bigg]\Bigg)^2
\end{align}

